Contrastive Learning for Implicit Social Factors in Social Media Popularity Prediction

On social media sharing platforms, some posts are inherently destined for popularity. Therefore, understanding the reasons behind this phenomenon and predicting popularity before post publication holds significant practical value. The previous work predominantly focuses on enhancing post content extraction for better prediction results. However, certain factors introduced by social platforms also impact post popularity, which has not been extensively studied. For instance, users are more likely to engage with posts from individuals they follow, potentially influencing the popularity of these posts. We term these factors, unrelated to the explicit attractiveness of content, as implicit social factors. Through the analysis of users' post browsing behavior (also validated in public datasets), we propose three implicit social factors related to popularity, including content relevance, user influence similarity, and user identity. To model the proposed social factors, we introduce three supervised contrastive learning tasks. For different task objectives and data types, we assign them to different encoders and control their gradient flows to achieve joint optimization. We also design corresponding sampling and augmentation algorithms to improve the effectiveness of contrastive learning. Extensive experiments on the Social Media Popularity Dataset validate the superiority of our proposed method and also confirm the important role of implicit social factors in popularity prediction. We open source the code at https://github.com/Daisy-zzz/PPCL.git.

==> sections/motivation.tex <==


\section{EXPLORATORY ANALYSIS}


To verify the rationality of the motivation, we perform a quantitative analysis of the widely-used Social Media Popularity Dataset (SMPD) ~\cite{wu2019smp}, which includes information about posts published on Flickr. In Figure ~\ref{fig:motistats-sub2}, we randomly select posts belonging to 20 Concepts. Different Concept labels in SMPD denote different content categories of posts. Then we present box plots of the chosen posts' popularity distributions, revealing obvious variations in the popularity of posts across different content categories and relative concentration of popularity within the same category, which validates factor CR. In Figure ~\ref{fig:motistats-sub1}, we choose the FollowerCount attribute to denote the user influence. Since the FollowerCount of different users varies greatly, we use $log_2$(FollowerCount) instead to draw the density plot. As we can see, the density reveals a more narrow distribution along the y-axis, indicating that users with similar influence tend to have posts that are relatively close in popularity, which validates factor UIS. In Figure ~\ref{fig:motistats-sub3}, we randomly select posts belonging to 20 users, the x-axis denotes userID.  It can be found that there are significant differences between the popularity distribution of posts by different users, and the high concentration of popularity among posts from the same user, which validates factor UI. These three observations effectively validate our hypothesis regarding the social factors influencing popularity. Note that this is only a preliminary verification of the motivation through quantitative analysis. We will later prove the effectiveness of the proposed social factors for popularity prediction through comprehensive experiments.

==> sections/preliminaries.tex <==
\section{preliminaries}
\subsection{Supervised Contrastive Learning}
To effectively utilize the label information, we utilize Supervised Contrastive Learning (SupCon) loss \cite{khosla2021supervised} as our training objectives. We first give the unsupervised contrastive loss formula for a pair of samples and then extend it to SupCon loss for all data. Given $N$ paired samples in a mini-batch $\mathcal{D}=\{\hat{x_i}\}_{i=1}^{2N}$, where $x_{2k}$ and $x_{2k-1}$ are positive pairs with related semantics $(k=1,...,N)$, denote $I=\{1,...,2N\}$ as the index of all samples, and $j(i)$ be the index of positive sample of $x_i$, the unsupervised contrastive objective of the pair $\{x_i, x_{j(i)}\}$ is:
\begin{equation}
    l(i) = -\log \frac{e^{\operatorname{sim}\left(\mathbf{f}_i, \mathbf{f}_{j(i)}\right) / \tau}}{\sum_{a \in A(i)} e^{\operatorname{sim}\left(\mathbf{f}_i, \mathbf{f}_a\right) / \tau}}
\end{equation}
where $f_i$ is the feature of $x_i$, $\tau$ is the temperature hyperparameter and $\operatorname{sim}(f_1, f_2)$ is the cosine similarity $\frac{f_1^T\cdot f_2}{\Vert f_1\Vert \cdot \Vert f_2\Vert}$, $A(i) = I \backslash \{i\}$ is all index except $i$ and then $A(i) \backslash \{j(i)\}$ are index of negative samples. The positive pairs are often chosen by different augmentations of the same source sample, and there is only one positive pair for each $x_i$. When it comes to the supervised scenario, we can use label information to construct more positive samples. Denote $P(i)=\{p \in A(i) | \hat{y_p} = \hat{y_i}\}$ as the samples which have the same label with $x_i$ in a mini-batch, the SupCon objective for all data in a mini-batch is:
\begin{equation} \label{eq:supcon}
    \mathcal{L}^{sup} = \sum_{i \in I} \frac{-1}{|P(i)|} \sum_{p \in P(i)} log \frac{e^{\operatorname{sim}\left(\mathbf{f}_i, \mathbf{f}_p\right) / \tau}}{\sum_{a \in A(i)} e^{\operatorname{sim}\left(\mathbf{f}_i, \mathbf{f}_a\right) / \tau}} 
\end{equation}
This supervised loss encourages the encoder to give closely aligned representations to all samples from the same class.

\subsection{Hierarchial Multi-label Contrastive Learning}
The posts from social media platforms usually have hierarchical labels to describe their content, thus we introduce Hierarchial Multi-label Contrastive Learning (HMCE) \cite{zhang2022use} loss, which extends Eq. ~\ref{eq:supcon} to the multi-label scenario. Let $L$ be the set of all label levels, and $l \in L$ is a level in the multi-label. Similar to SupCon, we denote $A(i) = I \backslash \{i\}$ is all index except $i$, and $P_l(i) = \{p \in A(I) | \hat{y}^l_p = \hat{y}^l_i\}$ is the samples which have the same label at level $l$ with $x_i$. The SupCon loss for a positive sample at level $l$ can be defined as:
\begin{equation} \label{eq:suppair}
L^{sup}(i, p_l^i) = log \frac{e^{\operatorname{sim}\left(\mathbf{f}_i, \mathbf{f}_p^l\right) / \tau}}{\sum_{a \in A(i)} e^{\operatorname{sim}\left(\mathbf{f}_i, \mathbf{f}_a\right) / \tau}}
\end{equation}
Then HMCE can be computed as:
\begin{equation} \label{eq:hmce}
   \mathcal{L}^{HMCE} = \sum_{l \in L} \frac{1}{|L|} \sum_{i \in I} \frac{-\lambda_l}{|P_l(i)|} \sum_{p_l \in P_l} \max \left(L^{\text {sup}}\left(i, p_l^i\right), L_{\max }^{\text {sup}}(l-1)\right)
\end{equation}
where $\lambda_l = F(l)$ is a controlling parameter that applies a fixed penalty for each level in the hierarchy, ensuring higher penalties to sample pairs constructed from higher levels in the hierarchy, because positive samples from lower levels may form negative pairs at higher levels. And
\begin{equation}\label{eq:supmax}
    L_{\max }^{\text {sup}}(l)=\max _{\left(i, p_l^i\right)} L^{\text {sup}}\left(i, p_l^i\right)
\end{equation}
is the hierarchical constraint that the loss between sample pairs from a higher level in the hierarchy will never be higher than the loss between pairs from a lower level, which stems from the observation that if a data point belongs to a class, it should also belong to its ancestors.
